QCD Processes in Few Nucleon Systems

One of the important issues of Quantum Chromodynamics (QCD) - the fundamental theory of strong interaction, is the understanding of the role of the quark-gluon interactions in the processes involving nuclear targets. One direction in such studies is to explore the onset of the quark gluon degrees of freedom in nuclear dynamics. The other direction is using the nuclear targets as a `micro-labs' in studies of the QCD processes involving protons and neutrons bound in the nucleus. In the proposed research, we work in both directions considering high energy photo- and electro-production reactions involving deuteron and $^3$He nuclei. In the first half of the research, we study the high energy break-up of the $^3$He nucleus, caused by a incoming photon, into a proton-deuteron pair at the large center of mass scattering angle. The main motivation of the research is the theoretical interpretation of recent experimental data which revealed the unprecedentedly large exponent $s^{-17}$, for the energy dependence of the differential cross section. In the present research, we extend the theoretical formalism of the hard QCD rescattering model to calculate energy and angular dependences of the absolute cross section of the $\gamma ^3\text{He}\rightarrow pd$ reaction in high momentum transfer limit. The second half of the research explores the deep-inelastic scattering of a polarized electron off the polarized deuteron and $^3$He nuclei, to explore the quark-gluon structure of polarized neutron. In this work, we developed a comprehensive theoretical framework for calculation of the all relevant nuclear effects that will allow the accurate extraction of the neutron data from deep-inelastic scattering involving deuteron and $^3$He targets.

==> 0/copyright.tex <==
\newpage
\vspace*{9cm}
\begin{center}
	\copyright \hspace{1pt} Copyright 2017 by Oswaldo Artiles\\
	All rights reserved.
\end{center}


==> 0/listFigures.tex <==
%\table of contents

\singlespacing


\hspace*{140pt} LIST OF FIGURES\\\\
FIGURE \hspace*{365pt} PAGE\\\\
\hspace*{12pt} 1.1 \hspace*{6pt} Lepton-nucleus inclusive scattering \dotfill  5\\\\
\hspace*{12pt} 1.2 \hspace*{6pt} Lepton-nucleus deep inelastic inclusive scattering regions \dotfill  8\\\\
\hspace*{12pt}  1.3 \hspace*{6pt} Theoretical predictions for the Fermi motion corrections of the bound nucleon\\
\hspace*{36pt} structure functions $F^N_2$ for iron. Figure from  \cite {Au83} \dotfill   10\\\\
\hspace*{12pt}  1.4 \hspace*{6pt} EMC experimental results for the ratio of the structure functions of iron nucleus\\
\hspace*{36pt}  and deuterium $(F^N_2(Fe)/F^N_2(D))$. Figure from  \cite {Au83} \dotfill  11\\\\
\hspace*{12pt}  1.5 \hspace*{6pt}Carbon EMC ratios for the highest $Q^2$ settings ($Q^2$ quoted at x = 0.75). Uncertain-
\hspace*{36pt}  ties are the combined statistical and point-to-point systematic. The solid curve is the\\
\hspace*{36pt}   SLAC fit to the Carbon EMC ratio. Figure from  \cite {Se09} \dotfill  12\\\\
\hspace*{12pt}  1.6 \hspace*{6pt} 2N and 3N scaling regions for nucleus A. Figure from Ref. \cite {Kim2}  \dotfill  12 \\\\
\hspace*{12pt}  1.7 \hspace*{6pt} The EMC slopes versus the SRC scale factors. Figure from Ref.
 \cite {LW1}   \dotfill  14  \\\\
\hspace*{12pt}  1.8 \hspace*{6pt} 2N and 3N SRC models for nuclear spectral functions  \dotfill  16\\\\
\hspace*{12pt}  2.1 \hspace*{6pt} Representation of the covariant Feynman amplitude through the sum of the time\\
\hspace*{36pt} ordered amplitudes. Panel (b) corresponds to the scenario in which first, the \\
\hspace*{36pt}  bound nucleon is resolved in the nucleus which interacts with the incoming probe\\
\hspace*{36pt}  $h$. In panel (c), initially, the incoming probe produces a $\bar N N$, anti-nucleon and\\
\hspace*{36pt} nucleon pair, with subsequent absorption of the $\bar N$ anti-nucleon in the nucleus. \dotfill   22\\\\
\hspace*{12pt}  2.2 \hspace*{6pt} Expansion of the nuclear spectral function into the contributions of the mean \\
\hspace*{36pt} field (a), the 2N (b) and the 3N (c) SRCs. For each case the initial nuclear tran-\\
\hspace*{36pt} sition vertices are different, corresponding to transition of $A\to N,A-1$; $A\to \\
\hspace*{36pt} NN,A-1$ and $A\to NNN,A-3$ for the mean field, the 2N and the 3N SRCs re-\\
\hspace*{36pt} spectively. The NN (b)  and NNN (c)  labels identify the 2N and the 3N SRCs with\\
 \hspace*{36pt} effective NN and NNN vertices  elaborated in the text \dotfill  27\\\\
\hspace*{12pt}  2.3 \hspace*{6pt} Diagram corresponding to the 3N SRC contribution to the nuclear  spectral func-\\
\hspace*{36pt} tions  \dotfill  29\\\\
\hspace*{12pt} 4.1 \hspace*{6pt} The momentum distribution of deuteron (s-wave: dot-dash, d-wave:dash) \dotfill   98\\\\
\hspace*{12pt} 4.2 \hspace*{6pt} Upper graph: Deuteron momentum distribution. Lower graph: Deuteron light-\\
\hspace*{36pt} front density matrix \dotfill    99\\\\
\hspace*{12pt} 4.3 \hspace*{6pt} Nuclear spectral function for $^9$Be in the nonrelativistic limit of  the VNA \dotfill  100\\\\
\hspace*{12pt} 4.4 \hspace*{6pt} Nuclear spectral function for $^{56}$Fe in the nonrelativistic limit of   the VNA  \dotfill   101\\\\
\hspace*{12pt} 4.5 \hspace*{6pt} Nuclear spectral function, with constant values of momentum for $^3$He and $^9$Be, in \\
\hspace*{36pt}   VNA and in the nonrelativistic limit of   the VNA\dotfill    102\\\\
\hspace*{12pt} 4.6 \hspace*{6pt} Nuclear spectral function for $^{9}$Be in light-front approximation, for $\tilde M^2_N = 0.5 \;\mathrm {GeV}^2$ \dotfill    103\\\\
\hspace*{12pt} 4.7 \hspace*{6pt} Nuclear spectral function for $^{197}$Au in light-front approximation, for $\tilde M^2_N = 0.2 \;\mathrm {GeV}^2$\\
\hspace*{36pt}   \dotfill    104\\\\
\hspace*{12pt} 4.8 \hspace*{6pt} SRC density matrix  for $^{9}$Be in light-front approximation \dotfill    105\\\\
\hspace*{12pt} 4.9 \hspace*{6pt} SRC density matrix  for $^{197}$Au in light-front approximation \dotfill    106\\\\
\hspace*{12pt} 4.10 \hspace*{0pt} SRC  momentum distribution  for proton in $^{3}$He, in VNA and in the nonrelativistic  \\
\hspace*{36pt}  limit of the VNA, the predictions in the nonrelativistic limit of the VNA are compa-   \\
\hspace*{36pt}  red to QMC calculations  \dotfill    110\\\\
\hspace*{12pt} 4.11 \hspace*{0pt} SRC momentum distribution for $^{8}$He in the nonrelativistic limit of the VNA compa-\\
\hspace*{36pt}  red to QMC calculations \dotfill    111\\\\
\hspace*{12pt} 4.12 \hspace*{0pt} SRC  momentum distribution  for neutron in $^{9}$Be, in VNA and in the nonrelativistic \\
\hspace*{36pt}  limit of the VNA, the predictions in the nonrelativistic limit of the VNA are compa-   \\
\hspace*{36pt} red to QMC calculations \dotfill    112\\\\
\hspace*{12pt} 4.13 \hspace*{0pt} SRC momentum distribution for $^{56}$Fe in the nonrelativistic limit of the VNA compa-\\
\hspace*{36pt} red to 2N SRC momentum distribution for proton in Ciofi/Simula [52] \dotfill    113\\\\
\hspace*{12pt} 4.14 \hspace*{0pt} SRC momentum distribution for $^{208}$Pb in VNA compared to predictions in the non-\\ 
\hspace*{36pt}  relativistic limit of the VNA \dotfill    113\\\\
\hspace*{12pt} 4.15 \hspace*{0pt} Momentum distribution for light nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions in the nonrelativistic limit of the VNA,  compared to the curve fitting ob-\\  
\hspace*{36pt}   tained with the mean field parameters in Table 4.3 and SRC parameters \;  in \; Table \\
\hspace*{36pt} 4.5 \dotfill    117\\\\
\hspace*{12pt} 4.16 \hspace*{0pt} Momentum distribution for heavy nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions  in the nonrelativistic limit of the VNA,   compared to the curve fitting ob-\\  
\hspace*{36pt}  tained with the mean field parameters in Table 4.4 and SRC parameters \;  in \; Table\\
 \hspace*{36pt} 4.6 \dotfill    118\\\\
\hspace*{12pt} 4.17 \hspace*{0pt} Momentum distribution for light nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions for VNA,  compared to the curve fitting obtained with  the mean field\\  
\hspace*{36pt}   parameters in Table 4.7 and SRC parameters  in Table 4.9 \dotfill    122\\\\
\hspace*{12pt} 4.18 \hspace*{0pt} Momentum distribution for heavy nuclei calculated with the SRC nuclear spectral\\
 \hspace*{36pt} functions for VNA,  compared to the curve fitting obtained with  the mean field\\  
\hspace*{36pt}  parameters in Table 4.8 and SRC parameters  in Table 4.10 \dotfill    123\\\\



==> 0/listTables.tex <==
%\table of contents

\singlespacing


\hspace*{140pt} LIST OF TABLES\\\\
TABLE \hspace*{370pt} PAGE\\\\
\hspace*{12pt} 4.1 \hspace*{6pt} 2N SRC parameters for light and heavy Nuclei (k$_F$ in GeV)\dotfill   107\\\\
\hspace*{12pt} 4.2 \hspace*{6pt} 3N SRC parameters for light and heavy nuclei \dotfill    108\\\\
\hspace*{12pt} 4.3 \hspace*{6pt} Parameters for the non-relativistic mean-field momentum distribution for light \\
\hspace*{36pt}   nuclei A $\le$ 12  \dotfill  115\\\\
\hspace*{12pt} 4.4 \hspace*{6pt} Parameters for the non-relativistic mean-field momentum distribution for heavy\\
\hspace*{36pt}  nuclei 16 $\le$ A $\le$ 208  \dotfill  115\\\\
\hspace*{12pt} 4.5 \hspace*{6pt} Parameters for the SRC momentum distribution in the nonrelativistic limit of the VNA\\
\hspace*{36pt}   for light nuclei A $\le$ 12  \dotfill    118\\\\
\hspace*{12pt} 4.6 \hspace*{6pt} Parameters for the SRC momentum distribution  in the nonrelativistic limit of the VNA  \\
\hspace*{36pt} for  heavy nuclei 16 $\le$ A $\le$ 208   \dotfill    118\\\\
\hspace*{12pt} 4.7 \hspace*{6pt} Parameters for  the mean-field  momentum distribution in VNA  for light nuclei A $\le$12 \\
 \hspace*{36pt}  \dotfill    119\\\\
\hspace*{12pt} 4.8 \hspace*{6pt} Parameters  for  the mean-field  momentum distribution in VNA  for heavy nuclei   \\
\hspace*{36pt} 16 $\le$ A $\le$ 208   \dotfill    119\\\\
\hspace*{12pt} 4.9 \hspace*{6pt} Parameters  for  the SRC  momentum distribution in VNA for light nuclei A $\le$12 
 \dotfill    120\\\\
\hspace*{12pt} 4.10 \hspace*{0pt} Parameters  for  the SRC  momentum distribution in VNA  for heavy nuclei  16 $\le$ A $\le$ 208\\
\hspace*{36pt}    \dotfill    120\\\\

